Efficient Policy Optimization in Robust Constrained MDPs with Iteration Complexity Guarantees

Constrained decision-making is essential for designing safe policies in real-world control systems, yet simulated environments often fail to capture real-world adversities. We consider the problem of learning a policy that will maximize the cumulative reward while satisfying a constraint, even when there is a mismatch between the real model and an accessible simulator/nominal model. In particular, we consider the robust constrained Markov decision problem (RCMDP) where an agent needs to maximize the reward and satisfy the constraint against the worst possible stochastic model under the uncertainty set centered around an unknown nominal model. Primal-dual methods, effective for standard constrained MDP (CMDP), are not applicable here because of the lack of the strong duality property. Further, one cannot apply the standard robust value-iteration based approach on the composite value function either as the worst case models may be different for the reward value function and the constraint value function. We propose a novel technique that effectively minimizes the constraint value function--to satisfy the constraints; on the other hand, when all the constraints are satisfied, it can simply maximize the robust reward value function. We prove that such an algorithm finds a policy with at most $\epsilon$ sub-optimality and feasible policy after $O(\epsilon^{-2})$ iterations. In contrast to the state-of-the-art method, we do not need to employ a binary search, thus, we reduce the computation time by at least 4x for smaller value of discount factor ($\gamma$) and by at least 6x for larger value of $\gamma$.

==> ideas.tex <==
\subsection{Better Rate}
To simplify the proof, we use some notations.
First, we denote
$\Phi(\pi_t)=\max\{J_{c_i}^{\pi}-b_i\}$ with $b_0=0$, and $J_{c_0}^{\pi}=J_{c_0}^{\pi}/\lambda$. 


We also use the following results from \cite{Epigraph}. 
\begin{lemma}
For any $\pi\in \Pi$, transition kernel $P:S\times A\rightarrow \Delta(S)$, the gradient is given by $(\nabla J_{c,P}(\pi))(s,a)=\dfrac{1}{1-\gamma}d_{P}^{\pi}(s)Q_{c,P}^{\pi}(s,a)$
\end{lemma}

 We also use the following result
% \begin{lemma}
% For any $i$
% \begin{align}
% J_{c_i}^{\pi,p}-J_{c_i}^{\pi^{\prime},p_{\prime}}=\sum_{s}d_{\rho}^{\pi_{t+1},p_{t+1}}(s)\sum_{a}(\pi_{t+1}(s,a)-\pi_t(s,a))q_{c_i}^{\pi_{t+1},p_t}
% \end{align}
% \end{lemma}

%We are now ready to obtain the result.

\begin{lemma}\label{lem:bregmen}
Let us assume that $i_t=\arg\max\{J_{c_i}^{\pi_t}-b_i\}$, then,
\begin{align}
\alpha_t\langle q_{s,i_t}^{\pi_t,p_t},\pi_{t+1,s}-y\rangle+B(\pi_{t+1,s},\pi_{t,s})\leq B(y,\pi_{t,s})-B(y,\pi_{t+1,s})
\end{align}
\end{lemma}
The above result follows from Bregmen divergence and the policy update.

We also use the following lemma proved in \cite{}.
\begin{lemma}\label{lem:performance_difference}
For any $\pi,\pi^{\prime}$, $p$, $c_i$, and $\rho$, we have
\begin{align}
J_{c_i,\rho}(\pi^{\prime},p)-J_{c_i,\rho}(\pi,p)=\dfrac{1}{1-\gamma}\sum_{s}d_{\rho}^{\pi,p}(s)\sum_a(\pi^{\prime}_{s,a}-\pi_{s,a})q_{s,a,c_i}^{\pi^{\prime},p}
\end{align}
\end{lemma}
Utilizing the above, we can conclude the following
\begin{lemma}

\end{lemma}
\begin{proof}
$i_t=\arg\max\{J_{c_i}^{\pi_t}-b_i\}$
\begin{align}
& \Phi(\pi_{t+1})-\Phi(\pi_{t})\geq J_{c_{i_t}}^{\pi_{t+1},p_t}-b_{i_t}-\max\{J_{c_i}^{\pi_t,p_t}-b_i\}\nonumber\\
& =\dfrac{1}{1-\gamma}\sum_{s}d_{\rho}^{\pi_{t+1},p_t}(s)\sum_a(\pi_{t
+1,s,a}-\pi_{t,s,a})q_{s,a,c_{i_t}}^{\pi_t,p_t}
\end{align}
\end{proof}
%%% Main results
\begin{theorem}
We have
\begin{align}
\Phi(\pi_t)-\Phi(\pi^*)\leq 
\end{align}

\end{theorem}

\begin{proof}
From Lemma~\ref{lem:bregmen}, by replacing $y=\pi^*$,
\begin{align}
\langle q_{s,i_t}^{\pi_t,p_t},\pi_{t,s}-\pi_s^*\rangle+\langle q_{s,i_t}^{\pi_t,p_t},\pi_{t+1,s}-\pi_{t,s}\rangle\leq \dfrac{1}{\alpha_t}B(\pi_s^*,\pi_{t,s})-\dfrac{1}{\alpha_t}B(\pi_s^*,\pi_{t+1,s})
\end{align}
where we use the fact that $B(\cdot)$ is non-negative.

Now,
\begin{align}\label{eq:modified_bregman}
& \Phi(\pi_t)-\Phi(\pi^*)=\max\{J_{c_0}^{\pi_t}-b_0,J_{c_i}^{\pi_t}-b_i\}-\max\{J_{c_0}^{\pi^*}-b_0,J_{c_i}^{\pi^*}-b_i\}\nonumber\\
& \leq J_{c_{i_t}}^{\pi_t,p_t}-J_{c_{i_t}}^{\pi^*,p_t}
%\leq H\max_{n,P}||\dfrac{d^{\pi_n^*,P}}{\mu}||_{\infty}\langle \pi_{t,s,a}-\pi^*_{s,a},q_{s,a}^{\pi_t,p_t}\rangle
\end{align}
where we use the fact that $i_t=\arg\max\{J_{c_i}^{\pi_t}-b_i\}$. Hence, using Lemma~\ref{lem:performance_difference}, we have
\begin{align}
J_{c_{i_t}}^{\pi_t,p_t}-J_{c_{i_t}}^{\pi^*,p_t}=\dfrac{1}{1-\gamma}\sum_{s}d_{\rho}^{\pi^*,p_t}(s)\sum_a(\pi_{t,s,a}-\pi^*_{s,a})q_{s,a,c_i}^{\pi_t,p}
\end{align}

Hence, applying (\ref{eq:modified_bregman}) we have
\begin{align}
\Phi(\pi_t)-\Phi(\pi^*)\leq [\dfrac{1}{1-\gamma}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_t}}\langle q_{s,i_t}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle+\dfrac{1}{\alpha_t}B(\pi^*,\pi_t)-\dfrac{1}{\alpha_t}B(\pi^*,\pi_{t+1})\nonumber\\
\leq \dfrac{1}{(1-\gamma)^2}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_t}}[\langle e,\pi_{t,s}-\pi_{s,t+1}\rangle]+\dfrac{1}{\alpha_t(1-\gamma)}(B(\pi^*,\pi_t)-B(\pi^*,\pi_{t+1}))
\end{align}
\textbf {The above inequality is not correct. Need to fix it}

Alternative, from Lemma~\ref{lem:bregmen}, we have
\begin{align}
&\Phi(\pi_t)-\Phi(\pi^*)\leq \nonumber\\
& [\dfrac{1}{1-\gamma}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_t}}\langle q_{s,i_t}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle+\dfrac{1}{\alpha_t}B(\pi^*,\pi_t)-\dfrac{1}{\alpha_t}B(\pi^*,\pi_{t+1})-\dfrac{1}{\alpha_t}B(\pi_{t+1},\pi_t)]
\end{align}

Now,
\begin{align}
& \langle q_{s,i_t}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle-\dfrac{1}{\alpha_t}B(\pi_{t+1},\pi_t)\leq ||q_{s,i_t}^{\pi_t,p_t}||_{\infty}||\pi_{t,s}-\pi_{t+1,s}||_1-\dfrac{1}{2\alpha_t}||\pi_{t,s}-\pi_{t+1,s}||_1^2\nonumber\\
& =\dfrac{-1}{2\alpha_t}(\alpha_t||q_{s,i_t}^{\pi_t,p_t}||_{\infty}-||\pi_{t,s}-\pi_{t+1,s}||_1)^2+\dfrac{\alpha_t}{2}||q_{s,i_t}^{\pi_t,p_t}||_{\infty}^2\nonumber\\
&\leq \dfrac{\alpha_t}{2}||q_{s,i_t}^{\pi_t,p_t}||_{\infty}^2
\end{align}

Hence, we have
\begin{align}
\Phi(\pi_t)-\Phi(\pi^*)\leq \dfrac{1}{1-\gamma}
\sum_{t=0}^{T-1}\mathbb{E}_{s \sim d_{\rho}^{\pi^*,p_t}}\alpha_t||q_{s,i}^{\pi_t,p_t}||_{\infty}^2\nonumber\\
+\dfrac{1}{\alpha_t(1-\gamma)}\mathbb{E}_{s \sim d_{\rho}^{\pi^*,p_t}}[B(\pi^*,\pi_t)-B(\pi^*,\pi_{t+1})]+T\epsilon_0\nonumber\\
\leq \dfrac{1}{(1-\gamma)}\sum_{t=0}^{T-1}\alpha_tS\dfrac{1}{(1-\gamma)^2}+\dfrac{1}{\alpha_0(1-\gamma)}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_0}}B(\pi^*,\pi_0)\nonumber\\
+\dfrac{1}{1-\gamma}\sum_{t=1}^{T-1}(\dfrac{1}{\alpha_t}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_t}}B(\pi^*,\pi_t)-\dfrac{1}{\alpha_{t-1}}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_{t-1}}}B(\pi^*,\pi_t))+T\epsilon_0
%\dfrac{1}{1-\gamma}\dfrac{1/(1-\gamma)^2}S\alpha_t+
\end{align}
We have
\begin{align}
\alpha_t\geq M\dfrac{\alpha_{t-1}}{1-\gamma}\geq \dfrac{\alpha_{t-1}}{1-\gamma}||d^{\pi^*,p_{t}}/\rho||_{\infty}\geq \alpha_{t-1}||\dfrac{d^{\pi^*,p_t}}{d^{\pi^*,p_{t-1}}}||_{\infty}\geq \alpha_{t-1}(\dfrac{d_{\rho}^{\pi^*,p_t}(s)}{d_{\rho}^{\pi^*,p_{t-1}}(s)})
\end{align}
hence, 
\begin{align}
    \dfrac{1}{\alpha_t}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_t}}B(\pi^*,\pi_t)-\dfrac{1}{\alpha_{t-1}}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_{t-1}}}B(\pi^*,\pi_t))\leq 0
\end{align}
Hence,
\begin{align}
\Phi(\pi_t)-\Phi(\pi^*)\leq \dfrac{1}{(1-\gamma)}\sum_{t=0}^{T-1}\alpha_tS\dfrac{1}{(1-\gamma)^2}+\dfrac{1}{\alpha_0(1-\gamma)}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_0}}B(\pi^*,\pi_0)+T\epsilon_0
\end{align}
Now, using $\alpha_t=\dfrac{M}{1-\gamma}\alpha_{t-1}$, and using $M\leq 1-\gamma$ thus, we have
\begin{align}
\Phi(\pi_t)-\Phi(\pi^*)\leq \dfrac{1}{(1-\gamma)}\dfrac{1}{1-M/(1-\gamma)}\alpha_0+\dfrac{1}{\alpha_0(1-\gamma)}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_0}}B(\pi^*,\pi_0)+T\epsilon_0
\end{align}
The result follows from the fact that $\alpha_0=\dfrac{1}{\sqrt{T}}$
%\end{align}


\textcolor{red}{
Using \citep[Lemma 2.6]{lin-first-order}, for any $\nu$,
\begin{align*}
0\leq \mathbb{E}_{s\sim \nu}\langle q_{s}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle &\leq \dfrac{1}{(1-\gamma)}\mathbb{E}_{s\sim d_{\nu}^{\pi_{t+1},p_{t+1}}}\langle q_{s}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle \\
&\leq \sum_{s} \nu_s \big(V^{\pi_t}(s) - V^{\pi_{t+1}}(s)\big).
\end{align*}
With Dirac $\nu$'s, we have $\big(V^{\pi_t}(s) - V^{\pi_{t+1}}(s)\big) \geq 0$ for all $s$.
From this and using $\nu = d_{\rho}^{\pi^*,p_{t}}$, 
\begin{align*}
0\leq \mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_t}}\langle q_{s}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle 
&\leq \sum_{s} d_{\rho,s}^{\pi^*,p_{t}} \big(V^{\pi_t}(s) - V^{\pi_{t+1}}(s)\big) \\
&\leq \sum_{s} \big(V^{\pi_t}(s) - V^{\pi_{t+1}}(s)\big).
\end{align*}
Summing over $t$, we have 
\begin{align*}
0\leq \sum_{t=0}^{T-1} \mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_t}}\langle q_{s}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle 
&\leq  \sum_{s} \sum_{t=0}^{T-1}  \big(V^{\pi_t}(s) - V^{\pi_{t+1}}(s)\big) = \sum_{s}  \big(V^{\pi_0}(s) - V^{\pi_{T}}(s)\big) \leq \frac{S}{1-\gamma}.
\end{align*}
Thanks for the proof. However, the issue is that here it will be $V_{c_{i_t}}^{\pi_t}-V_{c_{i_{t}}}^{\pi_{t+1}}$, hence, it would be difficult to do extend this idea here. However, it definitely fixes the original paper.\\ I see - it'll further require $i_t, i_{t+1}$ chaining argument. Thanks for pointing this. I see you already have an alternative proof. great.
}

Now, summing over $t$, we obtain
\begin{align}
\sum_t (\Phi(\pi_t)-\Phi(\pi^*))\leq \dfrac{1}{(1-\gamma)^2}\sum_{t=0}^{T-1}\mathbb{E}_{s \sim d_{\rho}^{\pi^*,p_t}}[\langle e,\pi_{s,t+1}-\pi_{s,t}\rangle]\nonumber\\
+\dfrac{1}{\alpha_t(1-\gamma)}\mathbb{E}_{s \sim d_{\rho}^{\pi^*,p_t}}[B(\pi^*,\pi_t)-B(\pi^*,\pi_{t+1})]+T\epsilon_0\nonumber\\
\leq \dfrac{1}{(1-\gamma)^2}\sum_{t=0}^{T-1}\mathbb{E}_{s \sim d_{\rho}^{\pi^*,p_t}}[\langle e,\pi_{s,t+1}-\pi_{s,t}]+\dfrac{1}{\alpha_0(1-\gamma)}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_0}}B(\pi^*,\pi_0)\nonumber\\
+\dfrac{1}{1-\gamma}\sum_{t=1}^{T-1}(\dfrac{1}{\alpha_t}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_t}}B(\pi^*,\pi_t)-\dfrac{1}{\alpha_{t-1}}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_{t-1}}}B(\pi^*,\pi_t))+T\epsilon_0
\end{align}
We have
\begin{align}
\alpha_t\geq M\dfrac{\alpha_{t-1}}{1-\gamma}\geq \dfrac{\alpha_{t-1}}{1-\gamma}||d^{\pi^*,p_{t}}/\rho||_{\infty}\geq \alpha_{t-1}||\dfrac{d^{\pi^*,p_t}}{d^{\pi^*,p_{t-1}}}||_{\infty}\geq \alpha_{t-1}(\dfrac{d_{\rho}^{\pi^*,p_t}(s)}{d_{\rho}^{\pi^*,p_{t-1}}(s)}
\end{align}

\end{proof}

\subsection{Modified Results}
\begin{align}\label{eq:modified_bregman}
& \Phi(\pi_t)-\Phi(\pi^*)=\max\{J_{c_0}^{\pi_t}-b_0,J_{c_i}^{\pi_t}-b_i\}-\max\{J_{c_0}^{\pi^*}-b_0,J_{c_i}^{\pi^*}-b_i\}\nonumber\\
& \leq J_{c_{i_t}}^{\pi_t,p_t}-J_{c_{i_t}}^{\pi^*,p_t}
%\leq H\max_{n,P}||\dfrac{d^{\pi_n^*,P}}{\mu}||_{\infty}\langle \pi_{t,s,a}-\pi^*_{s,a},q_{s,a}^{\pi_t,p_t}\rangle
\end{align}
Thus, from Performance Difference Lemma~\ref{lem:performance_difference}
\begin{align*}
& 0\leq \Phi(\pi_t)-\Phi(\pi^*)\leq J_{c_{i_t}}^{\pi_t,p_t}-J_{c_{i_t}}^{\pi^*,p_t}\\
& \leq \dfrac{1}{1-\gamma}\sum_sd_{\rho}^{\pi^*,p_t}\sum_a(\pi_{t,s,a}-\pi^*_{s,a})q_{s,a,c_{i_t}}^{\pi_t,p_t}
\end{align*}
Now, 
\begin{align}
\dfrac{d_{\rho}^{\pi^*,p_t}(s)}{\rho(s)}\leq ||\dfrac{d_{\rho}^{\pi^*,p_t}}{\rho}||_{\infty}\leq M
\end{align}
Hence,
\begin{align}
\Phi(\pi_t)-\Phi(\pi^*)\leq \dfrac{M}{1-\gamma}\sum_s\rho(s)\sum_a(\pi_{t,s,a}-\pi^*_{s,a})q_{s,a,c_{i_t}}^{\pi_t,p_t}
\end{align}
From Lemma~\ref{lem:bregmen}, we have
\begin{align}
&\Phi(\pi_t)-\Phi(\pi^*)\leq \nonumber\\
& [\dfrac{M}{1-\gamma}\mathbb{E}_{s\sim d_{\rho}}\langle q_{s,i_t}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle+\dfrac{1}{\alpha}B(\pi^*,\pi_t)-\dfrac{1}{\alpha}B(\pi^*,\pi_{t+1})-\dfrac{1}{\alpha}B(\pi_{t+1},\pi_t)]
\end{align}
Now,
\begin{align}
& \langle q_{s,i_t}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle-\dfrac{1}{\alpha}B(\pi_{t+1},\pi_t)\leq ||q_{s,i_t}^{\pi_t,p_t}||_{\infty}||\pi_{t,s}-\pi_{t+1,s}||_1-\dfrac{1}{2\alpha}||\pi_{t,s}-\pi_{t+1,s}||_1^2\nonumber\\
& =\dfrac{-1}{2\alpha}(\alpha_t||q_{s,i_t}^{\pi_t,p_t}||_{\infty}-||\pi_{t,s}-\pi_{t+1,s}||_1)^2+\dfrac{\alpha}{2}||q_{s,i_t}^{\pi_t,p_t}||_{\infty}^2\nonumber\\
&\leq \dfrac{\alpha}{2}||q_{s,i_t}^{\pi_t,p_t}||_{\infty}^2
\end{align}

Hence, we have
\begin{align}
& \sum_t(\Phi(\pi_t)-\Phi(\pi^*))\leq \dfrac{M}{1-\gamma}
\sum_{t=0}^{T-1}\mathbb{E}_{s \sim d_{\rho}}\alpha||q_{s,i}^{\pi_t,p_t}||_{\infty}^2\nonumber\\
& +\dfrac{M}{\alpha(1-\gamma)}\mathbb{E}_{s \sim d_{\rho}}[B(\pi^*,\pi_t)-B(\pi^*,\pi_{t+1})]+T\epsilon_0\nonumber\\
& \leq \dfrac{1}{(1-\beta)}\sum_{t=0}^{T-1}\alpha S\dfrac{1}{(1-\gamma)^2}+\dfrac{1}{\alpha(1-\beta)}\mathbb{E}_{s\sim d_{\rho}}B(\pi^*,\pi_0)+T\epsilon_0
%\dfrac{1}{1-\gamma}\dfrac{1/(1-\gamma)^2}S\alpha_t+
\end{align}
Hence,
\begin{align}
\sum_t(\Phi(\pi_t)-\Phi(\pi^*))\leq \dfrac{M}{1-\gamma}T\alpha S\dfrac{1}{(1-\gamma)^2\xi^2}+\dfrac{1}{\alpha(1-\beta)}\mathbb{E}_{s\sim d_{\rho}}B(\pi^*,\pi_0)+T\epsilon_0
\end{align}
Now, making $\pi_0=\dfrac{1}{|A|}$, and $\alpha=\dfrac{(1-\gamma)\xi}{\sqrt{TS}}$, we have
\begin{align}
\sum_t(\Phi(\pi_t)-\Phi(\pi^*))\leq \dfrac{M}{1-\gamma}\sqrt{ST}\log(|A|)\dfrac{1}{\sqrt{(\xi(1-\gamma))^2}}+T\epsilon_0
\end{align}
Hence,
\begin{align}
\Phi(\pi_t^*)-\Phi(\pi^*)\leq \dfrac{1}{T}\sum_t(\Phi(\pi_t)-\Phi(\pi^*))\leq \dfrac{\sqrt{S}}{(1-\beta)\sqrt{T(\xi(1-\gamma))^2}}+\epsilon_0
\end{align}
Hence, when $T=O(\dfrac{1}{(1-\gamma)^4\xi^2}S\log(|A|)(1/\epsilon^2))$ iteration, the above is bounded by $\epsilon$.

\subsection{Modified Result}\label{lem:modified}
\begin{align}\label{eq:modified_bregman}
& \Phi(\pi_t)-\Phi(\pi^*)=\max\{J_{c_0}^{\pi_t}-b_0,J_{c_i}^{\pi_t}-b_i\}-\max\{J_{c_0}^{\pi^*}-b_0,J_{c_i}^{\pi^*}-b_i\}\nonumber\\
& \leq J_{c_{i_t}}^{\pi_t,p_t}-J_{c_{i_t}}^{\pi^*,p_t}
%\leq H\max_{n,P}||\dfrac{d^{\pi_n^*,P}}{\mu}||_{\infty}\langle \pi_{t,s,a}-\pi^*_{s,a},q_{s,a}^{\pi_t,p_t}\rangle
\end{align}
Here, we use the following result from Lemma~\ref{alternate_performance}
\begin{align}
J_{c_{i_t}}^{\pi_t,p_t}-J_{c_{i_t}}^{\pi^*,p_t}\leq \dfrac{1}{1-\beta}\sum_{s}d_{\rho}^{\pi^*,p_0}(s)\sum_{a}(\pi_{t,s,a}-\pi^*_{s,a})q_{s,a,c_{i_t}}^{\pi_t,p_t}
\end{align}
From Lemma~\ref{lem:bregmen}, we have
\begin{align}
&\Phi(\pi_t)-\Phi(\pi^*)\leq \nonumber\\
& [\dfrac{1}{1-\beta}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_0}}\langle q_{s,i_t}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle+\dfrac{1}{\alpha}B(\pi^*,\pi_t)-\dfrac{1}{\alpha}B(\pi^*,\pi_{t+1})-\dfrac{1}{\alpha}B(\pi_{t+1},\pi_t)]
\end{align}
Now,
\begin{align}
& \langle q_{s,i_t}^{\pi_t,p_t},\pi_{t,s}-\pi_{t+1,s}\rangle-\dfrac{1}{\alpha}B(\pi_{t+1},\pi_t)\leq ||q_{s,i_t}^{\pi_t,p_t}||_{\infty}||\pi_{t,s}-\pi_{t+1,s}||_1-\dfrac{1}{2\alpha}||\pi_{t,s}-\pi_{t+1,s}||_1^2\nonumber\\
& =\dfrac{-1}{2\alpha}(\alpha_t||q_{s,i_t}^{\pi_t,p_t}||_{\infty}-||\pi_{t,s}-\pi_{t+1,s}||_1)^2+\dfrac{\alpha}{2}||q_{s,i_t}^{\pi_t,p_t}||_{\infty}^2\nonumber\\
&\leq \dfrac{\alpha}{2}||q_{s,i_t}^{\pi_t,p_t}||_{\infty}^2
\end{align}

Hence, we have
\begin{align}
\sum_t(\Phi(\pi_t)-\Phi(\pi^*))\leq \dfrac{1}{1-\beta}
\sum_{t=0}^{T-1}\mathbb{E}_{s \sim d_{\rho}^{\pi^*,p_0}}\alpha||q_{s,i}^{\pi_t,p_t}||_{\infty}^2\nonumber\\
+\dfrac{1}{\alpha(1-\beta)}\mathbb{E}_{s \sim d_{\rho}^{\pi^*,p_0}}[B(\pi^*,\pi_t)-B(\pi^*,\pi_{t+1})]+T\epsilon_0\nonumber\\
\leq \dfrac{1}{(1-\beta)}\sum_{t=0}^{T-1}\alpha S\dfrac{1}{(1-\gamma)^2}+\dfrac{1}{\alpha(1-\beta)}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_0}}B(\pi^*,\pi_0)+T\epsilon_0
%\dfrac{1}{1-\gamma}\dfrac{1/(1-\gamma)^2}S\alpha_t+
\end{align}
% We have
% \begin{align}
% \alpha_t\geq M\dfrac{\alpha_{t-1}}{1-\gamma}\geq \dfrac{\alpha_{t-1}}{1-\gamma}||d^{\pi^*,p_{t}}/\rho||_{\infty}\geq \alpha_{t-1}||\dfrac{d^{\pi^*,p_t}}{d^{\pi^*,p_{t-1}}}||_{\infty}\geq \alpha_{t-1}(\dfrac{d_{\rho}^{\pi^*,p_t}(s)}{d_{\rho}^{\pi^*,p_{t-1}}(s)})
% \end{align}
% hence, 
% \begin{align}
%     \dfrac{1}{\alpha_t}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_t}}B(\pi^*,\pi_t)-\dfrac{1}{\alpha_{t-1}}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_{t-1}}}B(\pi^*,\pi_t))\leq 0
% \end{align}
Hence,
\begin{align}
\sum_t(\Phi(\pi_t)-\Phi(\pi^*))\leq \dfrac{1}{(1-\beta)}T\alpha S\dfrac{1}{(1-\gamma)^2}+\dfrac{1}{\alpha(1-\beta)}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_0}}B(\pi^*,\pi_0)+T\epsilon_0
\end{align}
Now, making $\pi_0=\dfrac{1}{|A|}$, and $\alpha=\dfrac{(1-\gamma)}{\sqrt{TS}}$, we have
\begin{align}
\sum_t(\Phi(\pi_t)-\Phi(\pi^*))\leq \dfrac{1}{1-\beta}\sqrt{ST}\log(|A|)\dfrac{1}{\sqrt{(1-\gamma)^2}}+T\epsilon_0
\end{align}
Hence,
\begin{align}
\Phi(\pi_t^*)-\Phi(\pi^*)\leq \dfrac{1}{T}\sum_t(\Phi(\pi_t)-\Phi(\pi^*))\leq \dfrac{\sqrt{S}}{(1-\beta)\sqrt{T(1-\gamma)^2}}+\epsilon_0
\end{align}
Hence, when $T=O(\dfrac{1}{(1-\gamma)^2}S\log(|A|)(1/\epsilon^2))$ iteration, the above is bounded by $\epsilon$.

\subsection{Supporting Result}
\begin{lemma}\label{alternate_performance}
\begin{align}
\Phi(\pi)-\Phi(\pi^*)\leq \dfrac{1}{1-\beta}\mathbb{E}_{s\sim d_{\rho}^{\pi^*,p_0}}[\langle Q^{\pi,p}_{c_i},\pi_s-\pi^*]
\end{align}
where $i=\arg\max\{J_{c_i}^{\pi}-b_i\}$, and $p=\arg\max J_{c_i}^{\pi,P}$.
\end{lemma}
\begin{proof}
Let $i=\arg\max\{J_{c_i}^{\pi}-b_i\}$, and $p=\arg\max J_{c_i}^{\pi,P}$. Now, 
\begin{align}
\Phi(\pi)-\Phi(\pi^*)\leq J_{c_i}^{\pi,p}-J_{c_i}^{\pi^*,p}
\end{align}
We now bound the right-hand side.
\begin{align}
J_{c_i}^{\pi,p}-J_{c_i}^{\pi^*,p}=V^{\pi,p}_{c_i}(\rho)-\mathbb{E}_{s\sim \rho}\mathbb{E}_{\pi^*}[r(s,a)+\gamma\sum_{s^{\prime}}p(s^{\prime}|s,a)V^{\pi^*,p}_{c_i}(s^{\prime})]\nonumber\\
=\mathbb{E}_{s\sim \rho}\mathbb{E}_{a\sim \pi^*}[V_{c_i}^{\pi,p}(\rho)-r(s,a)+\gamma\sum_{s^{\prime}}p(s^{\prime}|s,a)V^{\pi,p}_{c_i}(s^{\prime})]\nonumber\\
-\mathbb{E}_{s\sim \rho}\mathbb{E}_{\pi^*}\gamma[\sum_{s^{\prime}}p(s^{\prime}|s,a)V^{\pi^*,p}_{c_i}(s^{\prime})-\sum_{s^{\prime}}p(s^{\prime}|s,a)V^{\pi,p}_{c_i}(s^{\prime})]\nonumber\\
= \sum_{s\sim \rho}\langle Q_{c_i}^{\pi},\pi-\pi^*\rangle-\gamma\mathbb{E}_{s\sim \rho}\mathbb{E}_{\pi^*}[\sum_{s^{\prime}}p(s^{\prime}|s,a)(V^{\pi^*,p}_{c_i}(s^{\prime})-V^{\pi,p}_{c_i}(s^{\prime}))]\nonumber\\
\leq \sum_{s\sim \rho}\langle Q_{c_i}^{\pi},\pi-\pi^*\rangle+\beta\mathbb{E}_{s\sim \rho}\mathbb{E}_{\pi^*}[\sum_{s^{\prime}}p_0(s^{\prime}|s,a)(V^{\pi}_{c_i}(s^{\prime})-V^{\pi^*}_{c_i}(s^{\prime}))]
\end{align}
where we use the fact that $V_{c_i}^{\pi,p}(s^{\prime})\geq V_{c_i}^{\pi^*,p}$ as $J_{c_i}^{\pi,p}-J_{c_i}^{\pi^*,p}\geq \Phi(\pi)-\Phi(\pi^*)\geq 0$.
By recursively, expanding we get the result.
\end{proof}
The assumption we need \textcolor{red}{can cite \citep{tamar2014scaling}}
\begin{assumption}
    There exists $\beta\in [0,1]$ such that $\gamma p(s^{\prime}|s,a)\leq \beta p_0(s^{\prime}|s,a)$ $\forall s^{\prime},a,$, and $p\in \mathcal{P}$.
\end{assumption}

\subsection{Removing the Assumption}
Let us consider the following assumption
\begin{align}
||q_{\pi,p_t}-q_{\pi^{\prime},p_t}||_{\infty}\leq L||\pi-\pi^{\prime}||_1
\end{align}


Using this, we can show the following
\begin{align}
\Phi(\pi_{t+1})-\Phi(\pi_t)= J_{i_{t+1}}^{\pi_{t+1},p_{t+1}}-J_{i_t}^{\pi_t,p_t}\leq J_{i_{t}}^{\pi_{t+1},p_{t}}-J_{i_t}^{\pi_t,p_t}+2L^{\prime}||\pi_t-\pi_{t+1}||
\end{align}
Note that $i_t$ is the best index for $\pi_t$. Due to the update
\begin{align}
|q_{s,a}^{\pi_{t+1},p_t}-q_{s,a}^{\pi_t,p_t}|\leq L||\pi_t-\pi_{t+1}||
\end{align}
Also note that
\begin{align}
\sum_s\rho(s)(\langle q_{s,a}^{\pi_t},\pi_t\rangle-\langle q_{s,a}^{\pi_{t+1}},\pi_{t+1}\rangle)\nonumber\\
\leq L^{\prime}||\pi_{t}-\pi_{t+1}||
\end{align}
Note that $p_t$ was the maximum index. Hence,
\begin{align}
J_{i_{t+1}}^{\pi_{t+1},p_{t+1}}\leq J_{i_{t+1}}^{\pi_t,p_{t+1}}+L^{\prime}||\pi_t-\pi_{t+1}||\leq J_{i_t}^{\pi_t,p_t}+L^{\prime}||\pi_t-\pi_{t+1}||\leq J_{i_t}^{\pi_{t+1},p_{t}}+2L^{\prime}||\pi_t-\pi_{t+1}||_1
\end{align}
Note that
\begin{align}
\langle q_{s,a}^{\pi_t},\pi_t\rangle-\langle q_{s,a}^{\pi_{t+1}},\pi_{t+1}\rangle\leq \langle q_{s,a}^{\pi_t}-q_{s,a}^{\pi_{t+1}},\pi_t\rangle-\langle q_{s,t}^{\pi_{t+1}},\pi_t-\pi_{t+1}\rangle\nonumber\\
\leq ||q_{s,a}^{\pi_t}-q_{s,a}^{\pi_{t+1}}||_{\infty}||\pi_t||_1+||q_{s,a}^{\pi_{t+1}}||_{\infty}||\pi_t-\pi_{t+1}||_1\nonumber\\
\leq L^{\prime}||\pi_t-\pi_{t+1}||_1
\end{align}



First, it is easy to see the following
\begin{lemma}
\begin{align}
\Phi(\pi_t)-\Phi(\pi^*)\leq M\min_{\pi^{\prime}_t}\langle \pi_t-\pi^{\prime}_t,Q^{\pi_t}_{c_i,p_t}\rangle
\end{align}
\end{lemma}
\begin{proof}


\end{proof}

Now, we have 
\begin{align}
\Phi(\pi_{t+1})-\Phi(\pi_t)\leq J_{i_{t}}^{\pi_{t+1},p_{t}}-J_{i_t}^{\pi_t,p_t}+2L^{\prime}||\pi_t-\pi_{t+1}||\leq 2||G(\pi)||+2L^{\prime}||\pi_t-\pi_{t+1}||\nonumber\\
\leq 
\end{align}

% Now,
% \begin{align}
% J_{i_{t}}^{\pi_{t+1},p_{t}}-J_{i_t}^{\pi_t,p_t}=\sum_s d_{\rho}^{\pi_t}\langle \pi_{t+1}-\pi_t,\nabla J_{i_t}^{\pi_t}\rangle
% \end{align}


Finally, we use the following results
\begin{align}
f(y)\leq f(x)+\langle \nabla f(x),y-x\rangle+\dfrac{L}||y-x||_2^2
\end{align}
to show that $J_{i_t}^{\pi_{t}}-J_{i_t}^{\pi_{t+1}}\geq \dfrac{1}{2L}||G(\pi_t)||_2^2$.

Finally, 
\begin{align}
    \min_{\pi^{\prime}}\langle \nabla J_{i_t}^{\pi_{t+1}},\pi_{t+1}-\pi^{\prime}\rangle\leq 2||G(\pi_t)||Diag
\end{align}
Now,
\begin{align}
\Phi(\pi_{t+1})-\Phi(\pi^*)\leq J_{i_{t+1}}^{\pi_{t+1},p_{t+1}}-J^*_{i_{t}}^{\pi^*,p_{t}}\nonumber\\
\leq J_{i_t}^{\pi_{t+1},p_{t}}-J_{i_t}^{\pi^*,p_t}\nonumber\\
\leq 2M||G(\pi_t)||Diag+
\end{align}


First, $\sum_{i}p(i)V_{i}^{\pi_{k+1},p_{k+1}}$, we will evaluate for each individual one

Now, we have
\begin{align}
\sum_i p_i(k)(V_i^{\pi_{k+1},p_{k+1}}-V_i^{\pi_k,p_k})+(p_i(k+1)-p_i(k))V_i^{\pi_{k+1},p_{k+1}}\geq -\gamma||\pi_{k+1}-\pi_{k}||H
\end{align}
\begin{proof}
\begin{align}
V_i^{\pi_{k+1},P_{k+1}}-V_i^{\pi_k,P_{k}}\geq V_{i}^{\pi_{k+1},P_{k}}-V_i^{\pi_k,P_{k}}\nonumber\\
=\dfrac{1}{1-\gamma}\sum_sd^{\pi_k,P_{k}}(s)\sum_a(\pi_{k+1}(a|s)-\pi_k(a|s))Q^{k+1}(s,a)\nonumber\\
=\dfrac{1}{1-\gamma}\sum_sd^{\pi_k,P_{k}}(s)\sum_a(\pi_{k+1}(a|s)-\pi_k(a|s))Q^{k}(s,a)+\dfrac{1}{1-\gamma}\sum_sd^{\pi_k,P_{k}}(s)\sum_a(\pi_{k+1}(a|s)-\pi_k(a|s))(Q^{k+1}(s,a)-Q^{k}(s,a)
\end{align}
Now, we have
\begin{align}
\sum_sd^{\pi_k,P_{k+1}}(s)\sum_a(\pi_{k+1}(a|s)-\pi_k(a|s))Q^{k}(s,a)\geq |S|||\pi_{k+1}-\pi_k||_1||Q||_{\infty}\nonumber\\
\sqrt{A}S||G_{\eta}||H
\end{align}
Now, combining all we have
\begin{align}
\Phi(\pi_{k+1})-\Phi(\pi_{k})\geq \eta\sqrt{A}S||G_{\eta}||H-\gamma ||\pi_k-\pi_{k+1}||-\theta H\nonumber\\
\Phi(\pi_K)-\Phi(\pi_0)\leq \sum_{k=1}^K \eta^2 AS||G_{\eta}||_2^2+K\theta\nonumber\\
-\dfrac{1}{1-\gamma}\leq \sum_{k=1}^K \eta^2 AS||G_{\eta}||_2^2+K\theta 
\end{align}
\begin{align}
\sum_{k=1}^K||G_{\eta}||_2^2\leq (\eta^2M^2)(1-\gamma)+H
\end{align}
\end{proof}


Now, we prove the result between $V^*$ and $V_k$, we will have
\begin{proof}
\begin{align}
V_{k+1}-V^*\leq (M+\eta A/(1-\gamma))||G_{\eta}||+\gamma\theta H
\end{align}
Then,
\begin{align}
\sum_k (V_{k+1}-V^*)^2\leq (M+\eta A/(1-\gamma))^2||G_{\eta}||_2^2+(\gamma\theta)^2H^2\nonumber\\
\leq (M+\eta A/(1-\gamma))(\eta-\gamma)+H^2\nonumber\\
(V_{k+1}-V^*)\leq \sqrt{C(1/\eta-1/\gamma)/K}
\end{align}
Make $\gamma=K^{-(1/3)}$, then, we have 
\begin{align}
(V_{k+1}-V^*)\leq \sqrt{C(K^{(-2/3)}}=O(K^{-1/3})
\end{align}
\end{proof}


New Proof Ideas:

\begin{align}
\Phi(\pi_{k+1})-\Phi(\pi_k)=\sum_i p(i,\pi_{k+1})V_i^{\pi_{k+1},p_{k+1}}-p(i,\pi_k)V_i^{\pi_k,p_k}\nonumber\\
\leq \sum_i p(i,\pi_{k})V_i^{\pi_{k+1},p_{k+1}}+(p(i,\pi_{k+1})-p(i,\pi_{k+1})V_i^{\pi_{k+1},p_{k+1}}-p(i,\pi_k)V_i^{\pi_k,p_k}\nounmber\\
\leq \sum_ip(i,\pi_k)(V_i^{\pi_{k+1},p_{k+1}}-V_i^{\pi_k,p_{k+1}})+||p(\pi_k)-p(\pi_{k+1}||_1H
\end{align}
We will bound the first term in the right-hand side. For each $i$
\begin{align}
V_i^{\pi_{k+1},p^i_{k+1}}-V_i^{\pi_k,p^i_{k}}\leq \sum_s d_{\rho}^{\pi_{k+1},p^i_{k+1}}(\pi_{k+1,s}-\pi_{k,s})Q_{i}^{\pi_k,p_k}\nonumber\\
\leq \dfrac{1}{M}\sum_s d_{\rho}^{\pi^*,p^i}(\pi_{k+1,s}-\pi_{k,s})Q_i^{\pi_k,p_k}
\end{align}
From the algorithm we have
\begin{align}
\langle p(i,\pi_k)Q_{i}^{\pi_k,p_k},\pi_{k+1}-\pi_k\rangle \nonumber\\
+\langle p(i,\pi_k)Q_{i}^{\pi_k,p_k},\pi_{k}-\pi^*\ranlge\leq \dfrac{1}{\alpha}B(\pi^*,\pi_k)-\dfrac{1}{\alpha} B(\pi^*,\pi_{k+1})
\end{align}

\begin{align}
\Phi(\pi_k)-\Phi(\pi^*)=\sum_i p(i,\pi_k)V_i^{\pi_k,p_k}-p(i,\pi^*)V_i^{\pi^*,p^*}\nonumber\\
=\sum_i (p(i,\pi_k)V_i^{\pi_k,p_k}-V_i^{\pi^*,p^*})+(p(i,\pi_k)-p(i,\pi^*))V_i^{\pi^*,p^*}\nonumber\\
\leq \sum_i (p(i,\pi_k)V_i^{\pi_k,p_k}-V_i^{\pi^*,p^*})+||p(i,\pi_k)-p(i,\pi^*)||_1H
\end{align}
Now, we have for any $i$
\begin{align}
V_i^{\pi_k,p_k}-V_i^{\pi^*,p^*}\leq \sum_sd_{\rho}^{\pi^*,p_k^i}(\pi_k-\pi^*)Q_i^{\pi_k,p_k}
\end{align}

\begin{align}
\pi_k^i
\end{align}
